Analyzing Oscillators using Describing Functions

In this manuscript, we discuss the use of describing functions as a systematic approach to the analysis and design of oscillators. Describing functions are traditionally used to study the stability of nonlinear control systems, and have been adapted for analyzing LC oscillators. We show that they can be applied to other categories of oscillators too, including relaxation and ring oscillators. With the help of several examples of oscillators from various physical domains, we illustrate the techniques involved, and also demonstrate the effectiveness and limitations of describing functions for oscillator analysis.

==> newcommands-colours.tex <==
% various colours
\definecolor{mylightgrey}{rgb}{0.6,0.6,0.6}
\definecolor{mydarkgrey}{rgb}{0.3,0.3,0.3}
\definecolor{mybrown}{rgb}{0.6,0.2,0}
\definecolor{mylightgreen}{rgb}{0,1,0}
\definecolor{mydarkgreen}{rgb}{0,0.5,0}
\definecolor{MyDarkGreen}{rgb}{0.0,0.4,0.0} % This is the color used for comments
\definecolor{myorange}{rgb}{1,0.4,0}
\definecolor{mypurple}{rgb}{0.8,0,0.8}
\definecolor{MyDarkRed}{rgb}{0.4,0.0,0.0} % This is the color used for strings


==> newcommands-comments-annotations.tex <==
% New commands for ignoring stuff from tex file, putting in comments and
% annotations
\newcommand{\ignore}[1]{}
\let\IGNORE=\ignore
%\newcommand{\comment}[1]{} % conflicts with something predefined
\newcommand{\COMMENT}[1]{}
\newcommand{\jrcomment}[1]{{\color{blue}#1}}
\newcommand{\agcomment}[1]{{\color{mydarkgreen}#1}}
\let\agc=\agcomment
\let\jc=\jrcomment
\newcommand{\redHL}[1]{{\color{red}\bf #1}}
\newcommand{\REDHL}[1]{{\color{red}\bf #1}}
\newcommand{\blueHL}[1]{\textbf{\color{blue}#1}}
\newcommand{\jsugg}[1]{\textit{\color{blue}#1}}
\newcommand{\jpvt}[1]{\textit{\color{red}#1}}
%\newcommand{\jsumm}[1]{{\color{blue}{{\uline{\textit{#1}}}}}}
\newcommand{\jsumm}[1]{\centerline{\color{blue}{{\uline{\textit{#1}}}}\\}}
\newcommand{\jkill}[1]{{\color{blue}\sout{#1}}}
\newcommand{\toputback}[1]{{\blueHL{PUT THIS BACK:} #1}}
\newcommand{\jemph}[1]{\textbf{\uline{#1}}}
\let\jnoteignored=\ignore
	
%\newcommand{\jnote}[1]{\textit{\color{blue}#1}}
%\newcommand{\jnote}[1]{\centerline{\color{mydarkgreen}{{\uline{\textit{#1}}}}\\}}
\newcommand{\jnote}[1]{% using fixme
	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
	\renewcommand{\fixmelogo}{}%
	\hspace*{-0.35em}\raisebox{0.7em}[\height][\depth]
            {\\\makebox[0em][l]{\fxnote{\tiny{\color{myred}JR: }
            \textit{\color{mydarkgreen}#1}}}}%
}
\let\jn=\jnote
\newcommand{\TOFIX}[1]{% using fixme
	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
	\renewcommand{\fixmelogo}{}%
	{\fxfatal{\bf\normalsize\textit{\color{myred}#1}}}%
}


==> newcommands-eg-ie-etc.tex <==
% eg, ie, etc, wrt, viz newcommands
\newcommand{\eg}{{\it e.g.\/}}
\newcommand{\ie}{{\it i.e.\/}}
\newcommand{\wrt}{{\it wrt}}
\newcommand{\viz}{{\it viz.\/}}
\newcommand{\vs}{{\it vs.\/}}
\newcommand{\aka}{{\it aka\/}}
\newcommand{\apriori}{{\it a priori}}
\newcommand{\etc}{\textit{etc.}}                                                
% etc defined so that there is only a single period after it if it is followed 
% by a period
% see: http://en.wikibooks.org/wiki/TeX/def                                      
% see: http://www.tug.org/pipermail/texhax/2004-July/002449.html                 
% see: http://en.wikibooks.org/wiki/TeX/if                                       
%\ifx \etc \undefined                                                             
%  %\def\myarg{#1}                                                                
%  %\def\myfullstop{.}                                                            
%  %\def\etc{#1}{\textit{etc} arg is ``\myarg'' \ifx\myarg\myfullstop\then.\else.#1\fi\/}
%  \def\etc#1{\textit{etc}\if#1..\else.#1\fi}                                     
%\fi                                                                              
%                        


==> newcommands-for-bibtex.tex <==
\newcommand{\BP}{({\textbf{Best Paper}})} % used in bibliography
\newcommand{\BPnom}{({\textbf{Best Paper Nomination}})} % used in bibliography
\newcommand{\IP}{({\textbf{Invited}})} % used in bibliography
\newcommand{\presenter}[1]{#1} % used in bibliography
\newcommand{\putDOI}[1]{#1}
%\newcommand{\putDOI}[1]{}
\newcommand{\DP}{\textbf{(Distinguished Paper)}}


==> newcommands-highlight-ignore.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% newcommands for ignoring, commenting, annotating, highlighting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ignore}[1]{}
\let\IGNORE=\ignore
%\newcommand{\comment}[1]{} % conflicts with something predefined
\newcommand{\COMMENT}[1]{}
\newcommand{\jrcomment}[1]{{\color{blue}#1}}
\let\jc=\jrcomment
\newcommand{\redHL}[1]{{\color{red}\bf #1}}
\newcommand{\REDHL}[1]{{\color{red}\bf #1}}
\newcommand{\blueHL}[1]{\textbf{\color{blue}#1}}
\newcommand{\jsugg}[1]{\textit{\color{blue}#1}}
\newcommand{\jpvt}[1]{\textit{\color{red}#1}}
%\newcommand{\jsumm}[1]{{\color{blue}{{\uline{\textit{#1}}}}}}
\newcommand{\jsumm}[1]{\centerline{\color{blue}{{\uline{\textit{#1}}}}\\}}
\newcommand{\jkill}[1]{{\color{blue}\sout{#1}}}
\newcommand{\toputback}[1]{{\blueHL{PUT THIS BACK:} #1}}
\newcommand{\jemph}[1]{\textbf{\uline{#1}}}
\newcommand{\jques}[1]{{\color{blue}#1?}}
\let\jnoteignored=\ignore
	
%\newcommand{\jnote}[1]{\textit{\color{blue}#1}}
\newcommand{\jnote}[1]{{\color{mydarkgreen}\textit{\uline{#1}}}}
\ignore{
    \newcommand{\jnote}[1]{% using fixme
    	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
    	\renewcommand{\fixmelogo}{}%
    	\hspace*{-0.35em}\raisebox{0.7em}[\height][\depth]
                {\\\makebox[0em][l]{\fxnote{\tiny{\color{myred}JR: }
                \textit{\color{mydarkgreen}#1}}}}%
    }
}
\let\jn=\jnote
\newcommand{\TOFIX}[1]{% using fixme
	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
	\renewcommand{\fixmelogo}{}%
	{\fxfatal{\bf\normalsize\textit{\color{myred}#1}}}%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END newcommands for ignoring, commenting, ....
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> newcommands-labels-refs.tex <==
% label and ref newcommands
% now mostly deprecated (but redefined and kept for backward compatibility) - move to \cref from the cleveref package
\crefname{algocf}{alg.}{algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{equation}{}{}
\Crefname{equation}{}{}

%DONE: xyzref{} should be able to handle multiple arguments so that you can
%reference multiple figures/equations at the same time -AG
%Now fixed with some package/command CREF.
\newcommand{\corrlabel}[1]{\label{corr:#1}}
\newcommand{\corrref}[1]{Corollary \ref{corr:#1}}
\newcommand{\assref}[1]{Assumption \ref{ass:#1}}
\newcommand{\asslabel}[1]{\label{ass:#1}}
%\newcommand{\eqnref}[1]{(\ref{eq:#1})}
%\newcommand{\eqnlabel}[1]{\label{eq:#1}}
\newcommand{\eqnlabel}[1]{\label{#1}}
\newcommand{\eqnref}[1]{\cref{#1}}
%\newcommand{\figlabel}[1]{\label{fig:#1}}
%\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figlabel}[1]{\label{#1}}
\newcommand{\figref}[1]{\cref{#1}}
\newcommand{\chaplabel}[1]{\label{chap:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\exampleref}[1]{Example~\ref{ex:#1}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\thlabel}[1]{\label{th:#1}}
\newcommand{\thref}[1]{Theorem~\ref{th:#1}}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem \ref{thm:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma \ref{lem:#1}}
\newcommand{\examplelabel}[1]{\label{ex:#1}}
\newcommand{\labexample}[1]{\label{example:#1}}
\newcommand{\refexample}[1]{Example{ }\ref{example:#1}}
\newcommand{\httpref}[1]{}
\let\el=\eqnlabel
\let\er=\eqnref


==> newcommands-math.tex <==
\newcommand{\ddt}[2]{{\frac{d}{d #2}\left. #1 \right.}}
\newcommand{\ddx}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\Ddx}[2]{{\frac{D}{d{#2}}\left[ #1 \right]}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\deq}{=}
\newcommand{\I}{I\left[\right]}
\newcommand{\ELL}[1]{L\left[#1\right]}
\newcommand{\w}{\omega}
\newcommand{\calD}{{\cal D}}
\renewcommand{\jmath}{j}
\newcommand{\Pinvt}{{P(t)}^{-1}}
\newcommand{\halmos}{\hskip\textwidth minus\textwidth \rule{6pt}{6pt}}
\newcommand{\calA}{{\cal A}}
\newcommand{\calAT}{{\cal A}^T}
\newcommand{\calL}{{\cal L}}
\newcommand{\calLadj}{\calL^\dagger}
\newcommand{\calR}{{\cal R}}
\newcommand{\Reals}{\Bbb{R}}
\newcommand{\Real}{\Bbb{R}}
\newcommand{\Safe}{\ensuremath{{\bf S}}}
\newcommand{\Pade}{{Pad\'e}}
\newcommand{\Complexes}{\Bbb{C}}
\newcommand{\HvecqLanc}{\Hvec^{(L)}_q}
\newcommand{\HvecqArn}{\Hvec^{(A)}_q}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\calDT}{{\cal D}^T}
\newcommand{\calCtil}{\tilde{\cal C}}
\newcommand{\calJtil}{\tilde{\cal J}}
\newcommand{\calDtil}{\tilde{\cal D}}
\newcommand{\JstarDphi}{J_{\Delta \phi}^*}
\newcommand{\Jstarphi}{J_{\phi}^*}
\newcommand{\vecbphi}{\vec b_{\phi}}
\newcommand{\vecbext}{\vec b_{\text{ext}}}
\newcommand{\phistarIdeal}{\phi_{\text{ideal}}^*}
\newcommand{\apdx}[1]{\appref{#1}} 
\newcommand{\delbydel}[2]{\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\delbydeln}[3]{\ensuremath{\frac{\partial^{{#1}}
{#2}}{\partial{#3}^{{#1}}}}}
\newcommand{\delbydelat}[3]{\ensuremath{\left. \frac{\partial
{#1}}{\partial {#2}} \right|_{{#3}}}}
\newcommand{\dee}{\ensuremath{\mathrm{d}}}
\newcommand{\dbyd}[2]{\ensuremath{\frac{\mathrm{d} {#1}}{\mathrm{d}
{#2}}}}
\newcommand{\dbydn}[3]{\ensuremath{\frac{\mathrm{d}^{{#1}}{#2}}
{\mathrm{d}{#3}^{{#1}}}}}
\newcommand {\dist}[1] {{{\rm dist}\left({#1}\right)}}
\def\Matrix#1{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\textdiag}{{\text{diag}}}
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
\newcommand{\khat}{\hat{k}}
\newcommand{\del}{\nabla}
\newcommand{\Rxx}{R_{\vec x \vec x}}
\newcommand{\Sxx}{S_{\vec x \vec x}}
\newcommand{\Snn}{S_{\vec n \vec n}}
\newcommand{\vecphi}{\vec \phi}
\newcommand{\Dphi}{\Delta \phi}
\newcommand{\vecDphi}{\vv{\Delta \phi}}
\newcommand{\dphi}{\delta \phi}
\newcommand{\vecdphi}{\vv{\delta \phi}}
\newcommand{\ah}{\alpha_g} % g for group
%\newcommand{\tDagger}{{\tilde t}}
\newcommand{\tDagger}{{t^{\!\dagger}}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\texthyphen}{\text{--}}

%The substack command can be used to produce a multi-line subscripts or superscripts:
%\sum_{\substack{0\le i\le m\\ 0<j<n}} P(i,j) produces a two-line subscript underneath the sum.
%A slightly more general form is the subarray environment which allows you to specify that each line should be left-aligned instead of centered, as here:
% \sum_{\begin{subarray}{l} i\in\Lambda\\ 0<j<n \end{subarray}} P(i,j) 

%\newcommand{\be}[1]{\begin{equation}\eqnlabel{#1}} % now moved to cleveref
\newcommand{\be}[1]{\begin{equation}\label{#1}}
\def\ee{\end{equation}}


==> newcommands-misc.tex <==
% Misc. commands
%\newcommand{\website}{http://www.eecs.berkeley.edu/\char126 jr/NOW-FT-Monograph/}
\newcommand{\figdir}{./figures}
\newcommand{\bibdir}{.}
\newif\ifjournalsub
\newcommand{\ifthen}[2]{\ifthenelse{#1}{#2}{}}
\newcommand{\iftr}[1]{\boolean{#1}}

\newcommand{\DAEtoFSM}{ABCD}
\newcommand{\Brangluin}{Brangluin}
\newcommand{\LTIMORrefs}{pillage1,FeFr95a,OdCePiTCAD98,PhDaSiDAC2002,PhSiPMTBRDATE2004}
\newcommand{\nonlinearMORrefs}{RoTVPTCAS99,ReWhTCAD2003,PhTCAD2003,DoRoTCADPWP2008,
                               GuRoICCAD2008maniMOR}
\newcommand{\MORrefs}{\LTIMORrefs,\nonlinearMORrefs}
\newcommand{\proposalAcronym}{THz-PHLOGON}
\newcommand{\website}{http://www.eecs.berkeley.edu/$\sim$jr/NOW-FT-Monograph/}
\newcommand{\PNJLIM}{\textsf{\small PNJLIM}}
%\newcommand{\MATLAB}{\textbf{MATLAB}$^{\texttrademark}$}
\newcommand{\MATLAB}{MATLAB$^\text{\textregistered}$}

% these are used in .bib files
\newcommand{\presenter}[1]{#1}
\newcommand{\BP}{\textbf{(Best Paper)}}
\newcommand{\BPnom}{\textbf{(Best Paper Nomination)}}
\newcommand{\IP}{\textbf{(Invited Paper)}}
\newcommand{\DP}{\textbf{(Distinguished Paper)}}

% various colours
\definecolor{mylightgrey}{rgb}{0.6,0.6,0.6}
\definecolor{mydarkgrey}{rgb}{0.3,0.3,0.3}
\definecolor{mybrown}{rgb}{0.6,0.2,0}
\definecolor{mylightgreen}{rgb}{0,1,0}
\definecolor{mydarkgreen}{rgb}{0,0.5,0}
\definecolor{MyDarkGreen}{rgb}{0.0,0.4,0.0} % This is the color used for comments
\definecolor{myorange}{rgb}{1,0.4,0}
\definecolor{mypurple}{rgb}{0.8,0,0.8}
\definecolor{MyDarkRed}{rgb}{0.4,0.0,0.0} % This is the color used for strings

%%%% misc formatting setup
\newlength{\colwidth}
\newcommand{\pswidthcoeff}{0.9}
\newcommand{\psheightcoeff}{0.6}
\newlength{\pgwid}
% make LaTeX less fussy about line breaks, so that it typsets inline 
% math without overflowing -- perhaps remove if it causes trouble.
\sloppy 
\setcounter{secnumdepth}{5}  % numbered \paragraph == \subsubsubsection
\pagenumbering{arabic}
%\renewcommand{\thepage} {Body--\arabic{page}}
\hyphenation{op-tical net-works semi-conduc-tor} % correct bad hyphenation here



==> newcommands-squeeze-spaces.tex <==
%%% tweaklist renewcommands
\newcommand{\modifiedListParamters}{
  \setlength{\topsep}{0pt}%
  \setlength{\itemsep}{-0.1em}
  \setlength{\partopsep}{0em}
  \setlength{\parsep}{0em}
  \setlength{\leftmargin}{1.1em}
  \setlength{\itemindent}{0.0em}
}
\renewcommand{\enumhook}{
  \modifiedListParamters
  \setlength{\itemindent}{0.2em}
}
\renewcommand{\itemhook}{
  \modifiedListParamters
}
\renewcommand{\descripthook}{
  \modifiedListParamters
  \setlength{\itemindent}{-1.0em}
}
%%% end tweaklist renewcommands

\ignore{not usually needed, but the definitions have useful info
		Space saving List environment for enumerations.

	\newcounter{myctr}
	\newenvironment{mylist}{\begin{list}{\arabic{myctr}.}
   		{\usecounter{myctr}
   		%\setlength{\topsep}{1mm}\setlength{\itemsep}{0.5mm}
   		\setlength{\topsep}{0.3mm}
   		\setlength{\itemsep}{0mm}
   		\setlength{\parsep}{0.3mm}
   		\setlength{\itemindent}{0mm}
   		\setlength{\partopsep}{0mm}
   		\setlength{\labelwidth}{15mm}
   		\setlength{\leftmargin}{4mm}
   		}
	}{\end{list}}

	\newenvironment{myitemize}{\begin{list}{$\bullet$}
	  \ignore{\setlength{\topsep}{0.8mm}\setlength{\itemsep}{0.25mm}}
	  {\setlength{\topsep}{1mm}\setlength{\itemsep}{0.25mm}
	  \setlength{\parsep}{0.1mm}
	  \setlength{\itemindent}{0mm}\setlength{\partopsep}{0mm}
	  \setlength{\labelwidth}{15mm}
	  \setlength{\leftmargin}{4mm}}
	}{\end{list}}
}

%%%% titlesec: squeezing whitespace between section headings
	\titlespacing{\section}{0pt}{*0}{*0.1} % {0pt} is indentation; {*0} is 
                                           % space above; {*0.5} is space below
	\titlespacing{\subsection}{0pt}{*0.1}{*0}
	\titlespacing{\subsubsection}{0pt}{*0.1}{*0}
%%%% end titlesec

%%%% squeezing whitespace in and around figures
    \floatsep=0em % space left between floats.
    \textfloatsep=0.5em % space between last top float or first bottom float and the text.
    \intextsep=0.5em % space left on top and bottom of an in-text float.
    %\dbltextfloatsep is \textfloatsep for 2 column output.
    %\dblfloatsep is \floatsep for 2 column output.
    \abovecaptionskip=0.2em % space above caption
    \belowcaptionskip=0.5em % space below caption
%%%% END squeezing whitespace in and around figures

\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{1pt}
  \setlength\belowdisplayskip{1pt}
  \setlength\abovedisplayshortskip{1pt}
  \setlength\belowdisplayshortskip{1pt}
}
\makeatother

%\newcommand{\mycaption}[1]{\caption{\small #1}}
\newcommand{\mycaption}[1]{\caption{\tiny #1}}

% for captions spacing
\captionsetup[table]{font={scriptsize},format=hang,indention=0em}     %% change 1.2 as you like
\captionsetup[figure]{font={scriptsize},format=hang,indention=0em}    %% change as you like
 %% or
 %% \captionsetup{font={stretch=1.2}}  %% this affects both figure and table

% replace Figure x in captions by Fig. x
%\renewcommand{\figurename}{Fig.} % doesn't work.
%but \usepackage[figurename=Fig.]{caption} in packages-headers.tex does work.


%\renewcommand{\baselinestretch}{1.5}
%\setstretch{1.5}

%\def\baselinestretch{0.8593}\large\normalsize - this form works locally?
%\renewcommand{\baselinestretch}{0.94} - this form works only in the preamble
%\renewcommand{\baselinestretch}{0.90}
%\renewcommand{\baselinestretch}{0.5}
%\linespread{0.5} % 0.5 -> 7 lines per inch; 0.9 -> a bit more than 6 lines 
%                 % per vertical inch
% \linespread{0.99}

% baselinestretch fixes for squeezing. See also linespread
%\def\ssp{\def\baselinestretch{0.95645}\large\normalsize} % "single space"
%\def\ssp{\def\baselinestretch{0.905}\large\normalsize} % "single space"
\def\ssp{\def\baselinestretch{0.9}\large\normalsize} % "single space"
\def\dsp{\def\baselinestretch{1.35}\large\normalsize} % "double space"
\ssp

% indent paragraphs less (saves space)
\parindent 	1em
% do not indent paragraphs (saves more space)
% \parindent 	0em
% adjust space between paragraphs (0em can obscure paragraph breaks)
\parskip 0.5em


==> newcommands-thm-env.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% theorem-like environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\EndProof{\hfill \quad \vrule width 1ex height 1ex depth 0pt  }
\newtheorem{corollary}{Corollary}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
%\newtheorem{illustration}{Illustration}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{notation}{Notation}
\newtheorem{theorem}{Theorem}
\newenvironment{sketch}{\noindent{\bf Sketch of Proof}:}{\halmos}
\newenvironment{conjecture}{\noindent{\bf Conjecture}: \em}{}
\newcommand{\numberedtheorem}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thetheorem
		\renewcommand{\thetheorem}{#1}
	}
	\begin{theorem}
	\ifthen{\not\equal{#2}{}}{
		\thmlabel{#2}
	}
	#3
	\end{theorem}
	\ifthen{\not\equal{#1}{}}{
		\let\thetheorem=\oof
		\addtocounter{theorem}{-1}
	}
}
\newcommand{\numberedlemma}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thelemma
		\renewcommand{\thelemma}{#1}
	}
	\begin{lemma}
	\ifthen{\not\equal{#2}{}}{
		\lemlabel{#2}
	}
	#3
	\end{lemma}
	\ifthen{\not\equal{#1}{}}{
		\let\thelemma=\oof
		\addtocounter{lemma}{-1}
	}
}


==> packages-headers.tex <==
%%%%%%%%%%%%%%%%%% PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%
\RequirePackage{times}
%\RequirePackage[usenames]{pstcol} 
\RequirePackage[usenames]{pstricks} 

% Graphics (figures/images etc.)
%\usepackage[pdftex]{graphicx}
\RequirePackage{graphicx} % supplies \includegraphics
\graphicspath{{./figures/}{./snapshots/}}
\DeclareGraphicsExtensions{.eps,.pdf,.jpeg,.png}

\RequirePackage{rotating}
\RequirePackage{indentfirst} 
\RequirePackage{color} 
%\RequirePackage{picins} 
\RequirePackage{bmpsize} 
\RequirePackage{epsfig} % good old way of including figures
\RequirePackage{eepic} 
\RequirePackage{subfigure} % put figures side-by-side
\RequirePackage{wrapfig} % wrap text around figures
\RequirePackage{picinpar} % alternative to wrapfig, less useful

% Math (symbols/equations etc.)
\usepackage{cancel}
\RequirePackage{amsmath,amssymb,amsthm,amsbsy,amsfonts,dotlessj} 
\RequirePackage{latexsym}
\RequirePackage{mathptm} % - AG (Don't like \mathcal{C} that this produces
\RequirePackage{mathptmx} % times (smaller) math fonts, greek characters also italicized
\RequirePackage{bm} % boldmath
\DeclareMathVersion{bold} 

% Formatting
\RequirePackage{multicol}
\RequirePackage{esvect} % defines \vv{}
\RequirePackage{ifthen}
\RequirePackage{etoolbox}
\RequirePackage{relsize}
\RequirePackage{soul}   % Provides \hl{some-text}
%\RequirePackage{showkeys} 
%\RequirePackage[final,notref]{showkeys} 
%\RequirePackage[top=0.8cm,bottom=0.8cm,left=0.8cm,right=0.8cm,nohead,nofoot]{geometry}
%\RequirePackage[top=1.2cm,bottom=1.3cm,left=1.2cm,right=1.2cm,nohead,nofoot]{geometry}

\usepackage[nolist,nohyperlinks]{acronym}
\RequirePackage{setspace}
\RequirePackage{moreverb}
\RequirePackage{ulem} % provides \uline
        \let\em=\it % ulem package redefines \em=\uline
\RequirePackage[sectionbib]{chapterbib}
\RequirePackage{fancyhdr}
\RequirePackage{array}
\RequirePackage{floatflt} % does (to some extent) work inside itemize environment %
                          % use \fltditem, see $LATEXDOCS/floatflt.pdf, esp. Sec 3.1
\RequirePackage{srcltx}
\RequirePackage{chemarrow}

% Utilities
\RequirePackage{tcolorbox}
\RequirePackage{fixme}
\RequirePackage[footnotesize,bf,figurename=Fig.,hang]{caption}
%\usepackage[scriptsize,hang,bf]{caption}
%\RequirePackage[hypertex]{hyperref} 
\RequirePackage{hyperref} 
%\definecolor{linkColor}{rgb}{0.1,0.1,0.8}
%\usepackage[colorlinks=true,bookmarks,pdfpagemode=UseOutlines,linkcolor=linkColor,citecolor=linkColor,pagecolor=blue,urlcolor=blue,pdftitle={Verification, Learning, Control},pdfauthor={Jaijeet Roychowdhury},plainpages=false]{hyperref}

\usepackage{./tweaklist} % allow changing of item spacings in standard itemize,
                         % enumerate, description environments
					     %%% tweaklist: compress lists. Also check out 
                         %%% \usepackage{mdwlist} (use itemize*, enumerate*, 
                         %%% description* with that)
                         % enumhook for the enumerate environment, itemhook for
                         % the itemize environment, and descripthook for the
                         % description environment.

\providecommand{\subparagraph}{} % needed for IEEEtran.cls (which does not define subparagraph); \providecommand checks if it is already defined
\RequirePackage[small,compact]{titlesec} % squeezing whitespace between section heading
\RequirePackage[square,sort&compress,numbers]{natbib} % needed for IEEEtran; but proposal.cls pulls it in automatically
%\RequirePackage{cite} % natbib doesn't like this
\RequirePackage{lipsum}
\RequirePackage{microtype}
\RequirePackage{url}
\RequirePackage{listings} % Required for insertion of code
\RequirePackage{multirow}
\RequirePackage{booktabs}
% load cleveref last, but before algorithm2e (which breaks cleveref)
\RequirePackage[compress,capitalise,noabbrev]{cleveref} % defines \cref, \Cref, etc; options are compress (don't sort), sort (don't compress), sort&compress (default), nosort (neither sort nor compress)
%\RequirePackage{algorithmic}
%\RequirePackage{algorithm}
%\RequirePackage[boxed,algoruled]{algorithm2e}
\RequirePackage[boxed,algoruled,linesnumbered,vlined,nofillcomment]{algorithm2e}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% fixme package setup
\fxsetup{ status=draft,
		  %author={\tiny JR},
	  	  layout=footnote,
		  layout=inline, % also try footnote or pdfnote
		  theme=color,
	  	  marginclue
}
\definecolor{mydarkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{myred}{rgb}{0.9,0.0,0.0}
%\definecolor{fxnote}{rgb}{0.8000,0.0000,0.0000}
\renewcommand{\englishlistfixmename}{List of changes needed}
% Decrease spacing between items in bib
\newcommand{\BIBdecl}{\setlength{\itemsep}{0.25 em}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Multi-column the bib
%\patchcmd{\thebibliography}
%  {\list}
%  {\begin{multicols}{2}\list}
%    {}
%    {}
%\appto{\endthebibliography}{\end{multicols}}

%------------------------------------------------------------------------------
%   CODE INCLUSION CONFIGURATION
%------------------------------------------------------------------------------

\lstloadlanguages{Matlab}
\lstset{language=Matlab,
        frame=single, % Single frame around code
        basicstyle=\scriptsize\ttfamily,
        % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
        keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{MyDarkGreen}\scriptsize, 
            % Comments are in small dark green courier font
        stringstyle=\color{MyDarkRed}, 
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=4, % 5 spaces per tab
        % 
        % Put standard functions not included in the default language here
        %morekeywords={rand},
        % Put function parameters here
        %morekeywords=[2]{on, off, interp},
        % Put user defined functions here
        %morekeywords=[3]{test},
        %
        morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
        % numbers=left, % Line numbers on left
        % firstnumber=1, % Line numbers start with line 1
        % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
        % stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
\newcommand{\matlabscript}[2]{
    \begin{itemize}
    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
    \end{itemize}
}


\input newcommands-colours
\input newcommands-highlight-ignore
\input newcommands-eg-ie-etc
\input newcommands-labels-refs
\input newcommands-math
\input newcommands-thm-env
\input newcommands-for-bibtex
\input newcommands-squeeze-spaces

